Parallelised Diffeomorphic Sampling-based Motion Planning

We propose Parallelised Diffeomorphic Sampling-based Motion Planning (PDMP). PDMP is a novel parallelised framework that uses bijective and differentiable mappings, or diffeomorphisms, to transform sampling distributions of sampling-based motion planners, in a manner akin to normalising flows. Unlike normalising flow models which use invertible neural network structures to represent these diffeomorphisms, we develop them from gradient information of desired costs, and encode desirable behaviour, such as obstacle avoidance. These transformed sampling distributions can then be used for sampling-based motion planning. A particular example is when we wish to imbue the sampling distribution with knowledge of the environment geometry, such that drawn samples are less prone to be in collisions. To this end, we propose to learn a continuous occupancy representation from environment occupancy data, such that gradients of the representation defines a valid diffeomorphism and is amenable to fast parallel evaluation. We use this to "morph" the sampling distribution to draw far fewer collision-prone samples. PDMP is able to leverage gradient information of costs, to inject specifications, in a manner similar to optimisation-based motion planning methods, but relies on drawing from a sampling distribution, retaining the tendency to find more global solutions, thereby bridging the gap between trajectory optimisation and sampling-based planning methods.

==> _env_vars.tex <==
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\definecolor{ashgrey}{rgb}{0.43, 0.5, 0.5}
\definecolor{yellow}{rgb}{1.0, 0.75, 0.0} %
\def\Cspace{\text{\emph{C-space}}\xspace}
\def\C{\ensuremath{C}\xspace}
\def\Cfree{\ensuremath{\C_\text{free}}\xspace}
\def\Cobs{\ensuremath{\C_\text{obs}}\xspace}
\def\Cobs{\ensuremath{\C_\text{obs}}\xspace}

\def\qinit{\ensuremath{q_\text{init}}\xspace}
\def\qtarget{\ensuremath{q_\text{target}}\xspace}

\newcommand*\workspace{\omega}

\def\star{\ensuremath{^{*}}}

\makeatletter

\def\rrt{\textsc{rrt}}%
\newcommand*\RRT{%
    \@ifstar{%
        \rrt\textsuperscript{*}\xspace%
    }{%
        \rrt\xspace%
    }}

\def\rrdt{\textsc{rr}{\smaller d}\textsc{t}}%
\newcommand*\RRdT{%
    \@ifstar{%
        \rrdt\textsuperscript{*}\xspace%
    }{%
        \rrdt\xspace%
    }}

\def\prm{\textsc{prm}}%
\newcommand*\PRM{%
    \@ifstar{%
        \prm\textsuperscript{*}\xspace%
    }{%
        \prm\xspace%
    }}

\makeatother



\newcommand*\Von[1][d]{\boldsymbol{V}\hspace{-.3em}\boldsymbol{on}_{#1}}
\newcommand*\Prob{\mathbb{P}}

\newcommand*\FailedSamSet{\mathcal{X}}
\newcommand*\SampleDist{\mathcal{Q}}
\newcommand*\SampleDistMul{\hat{\SampleDist{}}} %
\newcommand*\SampleDistQ{f_q}
\newcommand*{\SampleDistDelta}{\Delta_{\SampleDistMul}}

\newcommand*\State{\Theta}
\newcommand*\state{\theta}
\newcommand*\Observable{Q}

\newcommand*\ExpectedGain{\mathcal{V}_\text{gain}}

\newcommand*\param{\theta}

\newcommand*{\abs}[1]{\lvert#1\rvert}
\newcommand*{\norm}[1]{\lVert#1\rVert}

\newcommand*\vect[1]{\boldsymbol{#1}}
\newcommand*\given[1][]{\:#1\vert\:}



\makeatletter
\newcommand{\overrightsmallarrow}{\mathpalette{\overarrowsmall@\rightarrowfill@}}
\newcommand{\overarrowsmall@}[3]{%
  \vbox{%
    \ialign{%
      ##\crcr
      #1{\smaller@style{#2}}\crcr
      \noalign{\nointerlineskip}%
      $\m@th\hfil#2#3\hfil$\crcr
    }%
  }%
}
\def\smaller@style#1{%
  \ifx#1\displaystyle\scriptstyle\else
    \ifx#1\textstyle\scriptstyle\else
      \scriptscriptstyle
    \fi
  \fi
}
\makeatother

\newcommand*\Path[1]{\overrightsmallarrow{#1}}


\newcommand*\closureset[1]{\text{cl}(#1)}
\newcommand*\bLookOut[1]{%
    \ensuremath{\beta}\textsc{\footnotesize{-LookOut}}%
    \ifthenelse{\isempty{#1}}%
    {}{(#1)}%
}


\mathchardef\ordinarycolon\mathcode`\:
\mathcode`\:=\string"8000
\begingroup \catcode`\:=\active
  \gdef:{\mathrel{\mathop\ordinarycolon}}
\endgroup



